Accelerated Methods for Riemannian Min-Max Optimization Ensuring Bounded Geometric Penalties

In this work, we study optimization problems of the form $\min_x \max_y f(x, y)$, where $f(x, y)$ is defined on a product Riemannian manifold $\mathcal{M} \times \mathcal{N}$ and is $\mu_x$-strongly geodesically convex (g-convex) in $x$ and $\mu_y$-strongly g-concave in $y$, for $\mu_x, \mu_y \geq 0$. We design accelerated methods when $f$ is $(L_x, L_y, L_{xy})$-smooth and $\mathcal{M}$, $\mathcal{N}$ are Hadamard. To that aim we introduce new g-convex optimization results, of independent interest: we show global linear convergence for metric-projected Riemannian gradient descent and improve existing accelerated methods by reducing geometric constants. Additionally, we complete the analysis of two previous works applying to the Riemannian min-max case by removing an assumption about iterates staying in a pre-specified compact set.

==> definitions.tex <==
\usepackage{xparse}
\usepackage{xargs}

\makeatletter 
\def\Hy@raisedlink@left#1{%
    \ifvmode
        #1%
    \else
        \Hy@SaveSpaceFactor
        \llap{\smash{
        \begingroup
            \let\HyperRaiseLinkLength\@tempdima
            \setlength\HyperRaiseLinkLength\HyperRaiseLinkDefault
            \HyperRaiseLinkHook
        \expandafter\endgroup
        \expandafter\raise\the\HyperRaiseLinkLength\hbox{%
            \Hy@RestoreSpaceFactor
            #1%
            \Hy@SaveSpaceFactor
        }%
        }}
        \Hy@RestoreSpaceFactor
        \penalty\@M\hskip\z@ 
    \fi
}
\makeatother

\newcommand\newlink[2]{{\protect\hyperlink{#1}{\normalcolor #2}}}
\makeatletter
\newcommand\newtarget[2]{\Hy@raisedlink@left{\hypertarget{#1}{}}#2} 
\makeatother


\newcommand\linktoproof[1]{{\normalfont[{\hyperlink{proof:#1}{$\downarrow$}}]}}
\newcommand\linkofproof[1]{\textbf{of \cref{#1}. }\newtarget{proof:#1}}

\usepackage[bb=boondox]{mathalpha} 
\newcommand{\zeros}{\mathbb{0}} 
\newcommand\Hess{\operatorname{Hess}}

\newcommand{\RGD}{\newlink{def:acronym_riemannian_gradient_descent}{RGD}}
\newcommand{\PRGD}{\newlink{def:acronym_projected_riemannian_gradient_descent}{PRGD}}
\newcommand{\RAMMA}{\newlink{def:acronym_riemannian_accelerated_min_max_algorithm}{RAMMA}}
\newcommand{\RAMMAWC}{\newlink{def:acronym_riemannian_accelerated_min_max_algorithm-wc}{RAMMA-WC}}
\newcommand{\RIPPAWC}{\newlink{def:acronym_riemannian_inexact_proximal_point_algorithm}{RIPPA-WC}}
\newcommand{\RABR}{\newlink{def:acronym_riemannian_alternating_best_response}{RABR}}
\newcommand{\SCSC}{\newlink{def:acronym_strongly_g_convex_strongly_g_concave}{SCSC}}
\newcommand{\SCC}{\newlink{def:acronym_strongly_g_convex_g_concave}{SCC}}
\newcommand{\CC}{\newlink{def:acronym_g_convex_g_concave}{CC}}
\newcommand{\NCSC}{\newlink{def:acronym_non_g_convex_strongly_g_concave}{NCSC}}

\newcommand{\RCEG}{\newlink{def:acronym_riemannian_corrected_extra_gradient}{RCEG}}
\newcommand{\EG}{\newlink{def:acronym_extra_gradient}{EG}}


\newcommand{\bigoast}[1]{O^\ast( #1 )}
\newcommand{\bigoastl}[1]{O^\ast\left( #1 \right)}
\newcommand{\bigotilde}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}( #1 )}
\newcommand{\bigotildel}[1]{\newlink{def:big_o_tilde}{\widetilde{O}}\left( #1 \right)}
\newcommand{\bigomegatilde}[1]{\newlink{def:big_o_tilde}{\widetilde{\Omega}}( #1 )}


\newcommand{\riemacon}{\newlink{def:Riemacon_absolute_accuracy_SC}{\operatorname{RiemaconAbs}}}
\newcommand{\riemaconrel}{\newlink{def:Riemacon_relative_error_SC}{\operatorname{RiemaconRel}}}

\newcommand{\return}{\textbf{return}}

\let\oldmu\mu

\newcommand\Pii[1]{\newlink{def:euclidean_projection}{\Pi_{#1}}}

\let\olddelta\delta
\renewcommandx*\delta[2][1=, 2=, usedefault]{\newlink{def:delta}{\olddelta_{#1}^{#2}}}
\newcommand\deltad{\newlink{def:delta_without_subindex}{\olddelta}}


\let\oldzeta\zeta
\renewcommandx*\zeta[2][1=, 2=, usedefault]{\newlink{def:zeta}{\oldzeta_{#1}^{#2}}}
\newcommand\zetasq[1]{\newlink{def:zeta}{\oldzeta_{#1}^2}}
\newcommand\zetad{\newlink{def:zeta_without_subindex}{\oldzeta}}


\newcommandx*\kmin[1][1=, usedefault]{\newlink{def:minimum_sectional_curvature}{\kappa_{\min}^{#1}}}
\newcommandx*\kmax[1][1=, usedefault]{\newlink{def:maximum_sectional_curvature}{\kappa_{\max}^{#1}}}

\newcommandx*\kmint[1][1=, usedefault]{\tilde{\kappa}_{\min}^{#1}}
\newcommandx*\kmaxt[1][1=, usedefault]{\tilde{\kappa}_{\max}^{#1}}


\renewcommand\M{\newlink{def:M_manifold}{\mathcal{M}}}
\newcommand\MOnly{\mathcal{M}}
\newcommand\NN{\mathcal{N}}
\newcommand{\X}{\newlink{def:geodesically_convex_feasible_region}{\mathcal{X}}}
\newcommand{\XX}{\mathcal{X}} 
\newcommand{\Y}{\newlink{def:geodesically_convex_feasible_region_Y}{\mathcal{Y}}}
\renewcommand{\D}{\newlink{def:diameter_of_geodesically_convex_feasible_region}{D}}
\newcommand{\DExGr}{\newlink{def:diameter_of_geodesically_convex_region_for_extra_grad}{D}}
\newcommand{\Dcal}{\newlink{def:distance_to_saddle_extra_grad}{\mathcal{D}}}

\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\newlink{def:accuracy_epsilon}{\oldepsilon}}


\newcommand{\TOne}{\newlink{def:T_1}{T_1}}
\newcommand{\Ttwo}{\newlink{def:T_2}{T_2}}
\newcommand{\Tthree}{\newlink{def:T_3}{T_3}}
\newcommand{\Tfour}{\newlink{def:T_4}{T_4}}
\newcommand{\Tfive}{\newlink{def:T_5}{T_5}}

\newcommand{\epsilonone}{\newlink{def:epsilon_1}{\oldepsilon_1}}
\newcommand{\hatepsilonone}{\newlink{def:hat_epsilon_1}{\hat{\oldepsilon}_1}}
\newcommand{\epsilontwo}{\newlink{def:epsilon_2}{\oldepsilon_2}}
\newcommand{\epsilonthree}{\newlink{def:epsilon_3}{\oldepsilon_3}}
\newcommand{\hatepsilonthree}{\newlink{def:hat_epsilon_3}{\hat{\oldepsilon}_3}}
\newcommand{\epsilonfour}{\newlink{def:epsilon_4}{\oldepsilon_4}}
\newcommand{\epsilonfive}{\newlink{def:epsilon_5}{\oldepsilon_5}}

\let\oldGamma\Gamma
\renewcommand{\Gamma}[2]{\newlink{def:parallel_transport}{\oldGamma_{#1}^{#2}}}


\let\xiOnly\xi
\renewcommand{\xi}{\newlink{def:extra_geom_penalty_xi}{\xiOnly}}




\newcommandx*\proj[1][1=\X, usedefault]{\newlink{def:projection_operator}{\mathcal{P}_{#1}}}

\newcommand\expon[1]{\newlink{def:riemannian_exponential_map}{\operatorname{Exp}_{#1}}} 
\newcommand\exponinv[1]{\newlink{def:riemannian_exponential_map}{\operatorname{Log}_{#1}}} 

\newcommand{\Lips}{\newlink{def:Lipschitz_constant}{L_p}} 

\let\strikedL\L
\renewcommand{\L}{\newlink{def:max_of_Lx_Ly_and_Lxy}{L}} 
\newcommand{\Lsmooth}{\newlink{def:L_smooth}{L}} 
\newcommand{\Lx}{\newlink{def:smoothness_Lx}{L_x}} 
\newcommand{\Ly}{\newlink{def:smoothness_Ly}{L_y}} 
\newcommand{\Lxy}{\newlink{def:smoothness_Lxy}{L_{xy}}} 
\newcommand{\mux}{\newlink{def:strong_g_convexity_mu_x}{\oldmu_x}} 
\newcommand{\muy}{\newlink{def:strong_g_convexity_mu_y}{\oldmu_y}} 


\newcommand{\riemPlus}{\newlink{def:formal_riemannian_addition}{+}}
\newcommand{\riemMinus}{\newlink{def:formal_riemannian_subtraction}{-}}
\newcommand{\dist}{\newlink{def:distance}{d}}


\newcommand\f{\newlink{def:riemannian_function_f}{f}}


\newcommand\ball{\newlink{def:closed_ball}{\bar{B}}}
\newcommand\openball{B}

\newcommandx*\Ak[2][1=k, 2=, usedefault]{\newlink{def:integral_of_steps}{A_{#1}^{#2}}}
\newcommandx*\ak[2][1=k, 2=, usedefault]{\newlink{def:discrete_step}{a_{#1}^{#2}}}

\newcommand\Tansp[1]{\newlink{def:tangent_space}{T_{#1}}}


\newcommandx*\etak[2][1=k,2=, usedefault]{\newlink{def:MD_step_length}{\eta_{#1}^{#2}}}
\newcommandx*\tauk[1][1=k, usedefault]{\newlink{def:aux_tau_k}{\tau_{#1}}}
\newcommandx*\hk[1][1=k, usedefault]{\newlink{def:proximal_objective}{h_{#1}}}
\newcommandx*\yk[1][1=k, usedefault]{\newlink{def:iterate_y}{y_{#1}}}
\newcommandx*\ykast[1][1=k, usedefault]{\newlink{def:optimal_proximal_operator}{y_{#1}^{\ast}}}
\newcommandx*\xk[2][1=k,2=, usedefault]{\newlink{def:iterate_x}{x_{#1}^{#2}}}
\newcommandx*\xkp[2][1=k,2=, usedefault]{\newlink{def:iterate_xp}{x_{#1}'^{#2}}}
\newcommandx*\zy[2][1=k,2=k, usedefault]{\newlink{def:iterate_z_y}{z_{#1}^{y_{#2}}}}
\newcommandx*\zybar[2][1=k,2=k, usedefault]{\newlink{def:iterate_z_y_bar}{\bar{z}_{#1}^{y_{#2}}}}
\newcommandx*\zxbar[2][1=k,2=k, usedefault]{\newlink{def:iterate_z_x_from_z_y_bar}{z_{#1}^{x_{#2}}}}
\newcommandx*\zx[2][1=k,2=k, usedefault]{\newlink{def:iterate_z_x}{z_{#1}^{x_{#2}}}}
\newcommand\xInit{\newlink{def:initial_point}{x_0}}
\newcommand\xast{\newlink{def:x_part_of_optimum_saddle_point}{x^\ast}}
\newcommand\yast{\newlink{def:y_part_of_optimum_saddle_point}{y^\ast}}
\newcommand\xastg{\newlink{def:x_global_saddle}{\hat{x}^\ast}}
\newcommand\yastg{\newlink{def:y_global_saddle}{\hat{y}^\ast}}

\newcommandx*\vkx[1][1=k, usedefault]{\newlink{def:v_k_sup_x}{v_{#1}^{x}}}
\newcommandx*\vtkx[1][1=k, usedefault]{\newlink{def:v_tilde_k_sup_x}{\tilde{v}_{#1}^{x}}}
\newcommandx*\vtky[1][1=k, usedefault]{\newlink{def:v_tilde_k_sup_y}{\tilde{v}_{#1}^{y}}}

\newcommand\prox[1]{\newlink{def:prox}{\operatorname{prox}(#1)}}

\newcommand\indicator[1]{I_{#1}} 

\newcommandx*\gap[2][1=, 2=, usedefault]{\newlink{def:gap}{\operatorname{gap}}_{#2}(#1)}
\newcommandx*\gapx[2][1=, 2=, usedefault]{\newlink{def:gap_x}{\operatorname{gap}}_{#2}(#1)}
\newcommandx*\gapy[2][1=, 2=, usedefault]{\newlink{def:gap_y}{\operatorname{gap}}_{#2}(#1)}
\usepackage{mathabx} 
\newcommand\bargap[1]{\widebar{\operatorname{gap}}(#1)}

\newcommand\metric{\mathfrak{g}}
\newcommand\metrict{\tilde{\mathfrak{g}}}

\newcommand\etaEG{\newlink{def:learning_rate_eta_for_RCEG}{\eta}}

\newcommand\inj{\newlink{def:injectivity_radius}{\operatorname{inj}}}

\let\oldphi\phi
\renewcommand\phi{\newlink{def:function_max_over_y}{\oldphi}}


\newcommand\Deltazero{\newlink{def:initial_gap_of_phi}{\Delta_0}}

